Discontinuous Skeletal Gradient Discretisation Methods on polytopal meshes

In this work we develop arbitrary-order Discontinuous Skeletal Gradient Discretisations (DSGD) on general polytopal meshes. Discontinuous Skeletal refers to the fact that the globally coupled unknowns are broken polynomial on the mesh skeleton. The key ingredient is a high-order gradient reconstruction composed of two terms: (i) a consistent contribution obtained mimicking an integration by parts formula inside each element and (ii) a stabilising term for which sufficient design conditions are provided. An example of stabilisation that satisfies the design conditions is proposed based on a local lifting of high-order residuals on a Raviart-Thomas-N\'ed\'elec subspace. We prove that the novel DSGDs satisfy coercivity, consistency, limit-conformity, and compactness requirements that ensure convergence for a variety of elliptic and parabolic problems. Links with Hybrid High-Order, non-conforming Mimetic Finite Difference and non-conforming Virtual Element methods are also studied. Numerical examples complete the exposition.

==> exponential-dsgd <==
%------------------------------------------------------------------------------%
% Exponential test case, 1<p<2, DSGD
%------------------------------------------------------------------------------%

\begin{figure}\centering
  \begin{footnotesize}
    \ref{legend:exponential.tria:dsgd}
  \end{footnotesize}
  \vspace{0.25cm} \\
  %------------------------------------------------------------------------------%
  % Triangular mesh
  %------------------------------------------------------------------------------%
  \begin{minipage}{0.48\textwidth}\centering
    \begin{tikzpicture}[scale=0.70]
      \begin{loglogaxis}[
          legend columns=-1,
          legend to name=legend:exponential.tria:dsgd,
          legend style={/tikz/every even column/.append style={column sep=0.35cm}}
        ]
        % k=0
        \addplot[red,mark=*,mark options={solid},thick] table[x=meshsize,y=err_p]{plap-p-rt_0_mesh1.dat};
        % k=1
        \addplot[blue,mark=square*,mark options={solid},thick] table[x=meshsize,y=err_p]{plap-p-rt_1_mesh1.dat};
        % k=2
        \addplot[green!50!black,mark=diamond*,mark options={solid},thick] table[x=meshsize,y=err_p]{plap-p-rt_2_mesh1.dat};
        % k=3
        \addplot[brown,mark=triangle*,mark options={solid},thick] table[x=meshsize,y=err_p]{plap-p-rt_3_mesh1.dat};
        % k=4
        \addplot[violet,mark=star,mark options={solid},thick] table[x=meshsize,y=err_p]{plap-p-rt_4_mesh1.dat};

        \legend{$k=0$, $k=1$, $k=2$, $k=3$, $k=4$};
        
        % Slope triangles
        \logLogSlopeTriangle{0.875}{0.4}{0.1}{3/4}{black};
        \logLogSlopeTriangle{0.875}{0.4}{0.1}{3/2}{black};
        \logLogSlopeTriangle{0.875}{0.4}{0.1}{9/4}{black};
        \logLogSlopeTriangle{0.875}{0.4}{0.1}{3}{black};
        \logLogSlopeTriangle{0.875}{0.4}{0.1}{15/4}{black};
      \end{loglogaxis}
    \end{tikzpicture}
    \subcaption{Triangular, DSDG}
  \end{minipage}
  \begin{minipage}{0.48\textwidth}\centering
    \begin{tikzpicture}[scale=0.70]
      \begin{loglogaxis}
        % k=0
        \addplot[red,mark=*,mark options={solid},thick] table[x=meshsize,y=err_p]{plap-p_0_mesh1.dat};
        % k=1
        \addplot[blue,mark=square*,mark options={solid},thick] table[x=meshsize,y=err_p]{plap-p_1_mesh1.dat};
        % k=2
        \addplot[green!50!black,mark=diamond*,mark options={solid},thick] table[x=meshsize,y=err_p]{plap-p_2_mesh1.dat};
        % k=3
        \addplot[brown,mark=triangle*,mark options={solid},thick] table[x=meshsize,y=err_p]{plap-p_3_mesh1.dat};
        % k=4
        \addplot[violet,mark=star,mark options={solid},thick] table[x=meshsize,y=err_p]{plap-p_4_mesh1.dat};

        % Slope triangles
        \logLogSlopeTriangle{0.875}{0.4}{0.1}{3/4}{black};
        \logLogSlopeTriangle{0.875}{0.4}{0.1}{3/2}{black};
        \logLogSlopeTriangle{0.875}{0.4}{0.1}{9/4}{black};
        \logLogSlopeTriangle{0.875}{0.4}{0.1}{3}{black};
        \logLogSlopeTriangle{0.875}{0.4}{0.1}{15/4}{black};
      \end{loglogaxis}
    \end{tikzpicture}
    \subcaption{Triangular, HHO}
  \end{minipage}
  \vspace{0.25cm} \\
  %------------------------------------------------------------------------------%
  % Cartesian mesh
  %------------------------------------------------------------------------------%
  \begin{minipage}{0.48\textwidth}\centering
    \begin{tikzpicture}[scale=0.70]
      \begin{loglogaxis}
        % k=0
        \addplot[red,mark=*,mark options={solid},thick] table[x=meshsize,y=err_p]{plap-p-rt_0_mesh2.dat};
        % k=1
        \addplot[blue,mark=square*,mark options={solid},thick] table[x=meshsize,y=err_p]{plap-p-rt_1_mesh2.dat};
        % k=2
        \addplot[green!50!black,mark=diamond*,mark options={solid},thick] table[x=meshsize,y=err_p]{plap-p-rt_2_mesh2.dat};
        % k=3
        \addplot[brown,mark=triangle*,mark options={solid},thick] table[x=meshsize,y=err_p]{plap-p-rt_3_mesh2.dat};
        % k=4
        \addplot[violet,mark=star,mark options={solid},thick] table[x=meshsize,y=err_p]{plap-p-rt_4_mesh2.dat};
        
        % Slope triangles
        \logLogSlopeTriangle{0.875}{0.4}{0.1}{3/4}{black};
        \logLogSlopeTriangle{0.875}{0.4}{0.1}{3/2}{black};
        \logLogSlopeTriangle{0.875}{0.4}{0.1}{9/4}{black};
        \logLogSlopeTriangle{0.875}{0.4}{0.1}{3}{black};
        \logLogSlopeTriangle{0.875}{0.4}{0.1}{15/4}{black};
      \end{loglogaxis}
    \end{tikzpicture}    
    \subcaption{Cartesian, DSGD}
  \end{minipage}
  \begin{minipage}{0.48\textwidth}\centering
    \begin{tikzpicture}[scale=0.70]
      \begin{loglogaxis}
        % k=0
        \addplot[red,mark=*,mark options={solid},thick] table[x=meshsize,y=err_p]{plap-p_0_mesh2.dat};
        % k=1
        \addplot[blue,mark=square*,mark options={solid},thick] table[x=meshsize,y=err_p]{plap-p_1_mesh2.dat};
        % k=2
        \addplot[green!50!black,mark=diamond*,mark options={solid},thick] table[x=meshsize,y=err_p]{plap-p_2_mesh2.dat};
        % k=3
        \addplot[brown,mark=triangle*,mark options={solid},thick] table[x=meshsize,y=err_p]{plap-p_3_mesh2.dat};
        % k=4
        \addplot[violet,mark=star,mark options={solid},thick] table[x=meshsize,y=err_p]{plap-p_4_mesh2.dat};
        
        % Slope triangles
        \logLogSlopeTriangle{0.875}{0.4}{0.1}{3/4}{black};
        \logLogSlopeTriangle{0.875}{0.4}{0.1}{3/2}{black};
        \logLogSlopeTriangle{0.875}{0.4}{0.1}{9/4}{black};
        \logLogSlopeTriangle{0.875}{0.4}{0.1}{3}{black};
        \logLogSlopeTriangle{0.875}{0.4}{0.1}{15/4}{black};
      \end{loglogaxis}
    \end{tikzpicture}    
    \subcaption{Cartesian, HHO}
  \end{minipage}
  \vspace{0.25cm} \\
  %------------------------------------------------------------------------------%
  % Hexagonal mesh
  %------------------------------------------------------------------------------%
  \begin{minipage}{0.48\textwidth}\centering
    \begin{tikzpicture}[scale=0.70]
      \begin{loglogaxis}
        % k=0
        \addplot[red,mark=*,mark options={solid},thick] table[x=meshsize,y=err_p]{plap-p-rt_0_pi6_tiltedhexagonal.dat};
        % k=1
        \addplot[blue,mark=square*,mark options={solid},thick] table[x=meshsize,y=err_p]{plap-p-rt_1_pi6_tiltedhexagonal.dat};
        % k=2
        \addplot[green!50!black,mark=diamond*,mark options={solid},thick] table[x=meshsize,y=err_p]{plap-p-rt_2_pi6_tiltedhexagonal.dat};
        % k=3
        \addplot[brown,mark=triangle*,mark options={solid},thick] table[x=meshsize,y=err_p]{plap-p-rt_3_pi6_tiltedhexagonal.dat};
        % k=4
        \addplot[violet,mark=star,mark options={solid},thick] table[x=meshsize,y=err_p]{plap-p-rt_4_pi6_tiltedhexagonal.dat};
        
        % Slope triangles
        \logLogSlopeTriangle{0.875}{0.4}{0.1}{3/4}{black};
        \logLogSlopeTriangle{0.875}{0.4}{0.1}{3/2}{black};
        \logLogSlopeTriangle{0.875}{0.4}{0.1}{9/4}{black};
        \logLogSlopeTriangle{0.875}{0.4}{0.1}{3}{black};
        \logLogSlopeTriangle{0.875}{0.4}{0.1}{15/4}{black};
      \end{loglogaxis}
    \end{tikzpicture}    
    \subcaption{Hexagonal, DSGD}
  \end{minipage}
    \begin{minipage}{0.48\textwidth}\centering
    \begin{tikzpicture}[scale=0.70]
      \begin{loglogaxis}
        % k=0
        \addplot[red,mark=*,mark options={solid},thick] table[x=meshsize,y=err_p]{plap-p_0_pi6_tiltedhexagonal.dat};
        % k=1
        \addplot[blue,mark=square*,mark options={solid},thick] table[x=meshsize,y=err_p]{plap-p_1_pi6_tiltedhexagonal.dat};
        % k=2
        \addplot[green!50!black,mark=diamond*,mark options={solid},thick] table[x=meshsize,y=err_p]{plap-p_2_pi6_tiltedhexagonal.dat};
        % k=3
        \addplot[brown,mark=triangle*,mark options={solid},thick] table[x=meshsize,y=err_p]{plap-p_3_pi6_tiltedhexagonal.dat};
        % k=4
        \addplot[violet,mark=star,mark options={solid},thick] table[x=meshsize,y=err_p]{plap-p_4_pi6_tiltedhexagonal.dat};
        
        % Slope triangles
        \logLogSlopeTriangle{0.875}{0.4}{0.1}{3/4}{black};
        \logLogSlopeTriangle{0.875}{0.4}{0.1}{3/2}{black};
        \logLogSlopeTriangle{0.875}{0.4}{0.1}{9/4}{black};
        \logLogSlopeTriangle{0.875}{0.4}{0.1}{3}{black};
        \logLogSlopeTriangle{0.875}{0.4}{0.1}{15/4}{black};
      \end{loglogaxis}
    \end{tikzpicture}    
    \subcaption{Hexagonal, HHO}
  \end{minipage}
  \vspace{0.25cm} \\
  % Locally refined mesh
  \begin{minipage}{0.48\textwidth}\centering
    \begin{tikzpicture}[scale=0.70]
      \begin{loglogaxis}
        % k=0
        \addplot[red,mark=*,mark options={solid},thick] table[x=meshsize,y=err_p]{plap-p-rt_0_mesh3.dat};
        % k=1
        \addplot[blue,mark=square*,mark options={solid},thick] table[x=meshsize,y=err_p]{plap-p-rt_1_mesh3.dat};
        % k=2
        \addplot[green!50!black,mark=diamond*,mark options={solid},thick] table[x=meshsize,y=err_p]{plap-p-rt_2_mesh3.dat};
        % k=3
        \addplot[brown,mark=triangle*,mark options={solid},thick] table[x=meshsize,y=err_p]{plap-p-rt_3_mesh3.dat};
        % k=4
        \addplot[violet,mark=star,mark options={solid},thick] table[x=meshsize,y=err_p]{plap-p-rt_4_mesh3.dat};
        
        % Slope triangles
        \logLogSlopeTriangle{0.875}{0.4}{0.1}{3/4}{black};
        \logLogSlopeTriangle{0.875}{0.4}{0.1}{3/2}{black};
        \logLogSlopeTriangle{0.875}{0.4}{0.1}{9/4}{black};
        \logLogSlopeTriangle{0.875}{0.4}{0.1}{3}{black};
        \logLogSlopeTriangle{0.875}{0.4}{0.1}{15/4}{black};
      \end{loglogaxis}
    \end{tikzpicture}    
    \subcaption{Locally refined, DSGD}
  \end{minipage}
    \begin{minipage}{0.48\textwidth}\centering
    \begin{tikzpicture}[scale=0.70]
      \begin{loglogaxis}
        % k=0
        \addplot[red,mark=*,mark options={solid},thick] table[x=meshsize,y=err_p]{plap-p_0_mesh3.dat};
        % k=1
        \addplot[blue,mark=square*,mark options={solid},thick] table[x=meshsize,y=err_p]{plap-p_1_mesh3.dat};
        % k=2
        \addplot[green!50!black,mark=diamond*,mark options={solid},thick] table[x=meshsize,y=err_p]{plap-p_2_mesh3.dat};
        % k=3
        \addplot[brown,mark=triangle*,mark options={solid},thick] table[x=meshsize,y=err_p]{plap-p_3_mesh3.dat};
        % k=4
        \addplot[violet,mark=star,mark options={solid},thick] table[x=meshsize,y=err_p]{plap-p_4_mesh3.dat};
        
        % Slope triangles
        \logLogSlopeTriangle{0.875}{0.4}{0.1}{3/4}{black};
        \logLogSlopeTriangle{0.875}{0.4}{0.1}{3/2}{black};
        \logLogSlopeTriangle{0.875}{0.4}{0.1}{9/4}{black};
        \logLogSlopeTriangle{0.875}{0.4}{0.1}{3}{black};
        \logLogSlopeTriangle{0.875}{0.4}{0.1}{15/4}{black};
      \end{loglogaxis}
    \end{tikzpicture}    
    \subcaption{Locally refined, HHO}
  \end{minipage}
  \caption{Error v. h, exponential test case, $p=\frac34$. For the DSGD method (left) the error is measured by $\norm[L^p(\Omega)^d]{\grD[h](\Ih u-\uu)}$, for the HHO method (right) by $\norm[1,p,h]{\Ih u-\uu}$.\label{fig:exponential:dsgd}}
\end{figure}

